PBR3DGen: A VLM-guided Mesh Generation with High-quality PBR Texture

Generating high-quality physically based rendering (PBR) materials is important to achieve realistic rendering in the downstream tasks, yet it remains challenging due to the intertwined effects of materials and lighting. While existing methods have made breakthroughs by incorporating material decomposition in the 3D generation pipeline, they tend to bake highlights into albedo and ignore spatially varying properties of metallicity and roughness. In this work, we present PBR3DGen, a two-stage mesh generation method with high-quality PBR materials that integrates the novel multi-view PBR material estimation model and a 3D PBR mesh reconstruction model. Specifically, PBR3DGen leverages vision language models (VLM) to guide multi-view diffusion, precisely capturing the spatial distribution and inherent attributes of reflective-metalness material. Additionally, we incorporate view-dependent illumination-aware conditions as pixel-aware priors to enhance spatially varying material properties. Furthermore, our reconstruction model reconstructs high-quality mesh with PBR materials. Experimental results demonstrate that PBR3DGen significantly outperforms existing methods, achieving new state-of-the-art results for PBR estimation and mesh generation. More results and visualization can be found on our project page: https://pbr3dgen1218.github.io/.

==> figs_tex/qualitative_comparison_reconstruction_text2mesh.tex <==
\begin{figure*}[thbp]
%\setlength{\abovecaptionskip}{ -8 pt}
\centering
  \includegraphics[width=0.88\linewidth]{figs/LRM_Comparison-text2mesh.pdf}
  \vspace{-0.4cm}
\caption{ Qualitative comparison of the generated 3D assets with other methods on Text2mesh. }
\label{fig:LRM_Comparison_text2mesh}
\vspace{-0.2cm}
\end{figure*}

==> rebuttal_figs_tex/FID_objaverse_dataset.tex <==
\vspace{-0.4cm}
\begin{table}[htbp]
\centering
\caption{FID comparison on Objaverse [10] dataset.}
\footnotesize % 缩小字体
\label{tab:fid_comparison}
\vspace{-0.3cm}
\begin{adjustbox}{max width=0.75\textwidth, center} % 控制表格宽度为页面宽度的85%
% \small
\begin{tabular}{@{}lcc@{}}
\toprule
\textbf{Method} & \textbf{Albedo(FID$\downarrow$)} & \textbf{RGB(FID$\downarrow$)} \\ 
\midrule
Ours & \textbf{50.63} & \textbf{49.37} \\
SF3D & 57.67 & 55.36 \\
PrimX & 78.55 & 68.49 \\
\bottomrule
\label{re_table:FID_obj}
\vspace{-0.65cm}
\end{tabular}
\end{adjustbox}
\end{table}

==> rebuttal_figs_tex/distibution_comparison_with_intrinsicAny.tex <==
\begin{table}[h!]
\centering
\caption{Comparison of distribution on PSNR and MSE between IntrinsicAnything and Ours.} % 将 caption 放在表格上方
\vspace{-0.3cm}
\label{tab:results}
\begin{adjustbox}{width=0.4\textwidth} % 调整表格宽度
\begin{tabular}{lccccc}
\toprule
{Method} & \multicolumn{2}{c}{PSNR} & \multicolumn{2}{c}{MSE} \\
\cmidrule(lr){2-3} \cmidrule(lr){4-5}
 & Mean ($\uparrow$) & Std ($\downarrow$) & Mean ($\downarrow$) & Std ($\downarrow$) \\
\midrule
IntrinsicAnything & 16.77522 & 0.29651 & 0.03195 & 0.00181 \\
Ours & \textbf{18.18618} & \textbf{0.27967} & \textbf{0.02379} & \textbf{0.00125} \\
\bottomrule
\label{re_table:robustness}
\end{tabular}
\end{adjustbox}
\end{table}


==> rebuttal_figs_tex/spec_light_eval.tex <==
\begin{table}[h]
\centering
\vspace{-0.3cm}
\caption{Quantitative evaluation of illumination model}
\vspace{-0.3cm}
\footnotesize % 缩小字体
\begin{tabular}{@{}lcccc@{}}
\toprule
\textbf{Metric} & \textbf{MSE} & \textbf{PSNR (dB)} & \textbf{SSIM} & \textbf{LPIPS} \\
\midrule
Ours & 0.0197 & 18.98 & 0.8752 & 0.0001 \\
\bottomrule
\end{tabular}
\end{table}
